Jellyfish: Networking Data Centers Randomly

Industry experience indicates that the ability to incrementally expand data centers is essential. However, existing high-bandwidth network designs have rigid structure that interferes with incremental expansion. We present Jellyfish, a high-capacity network interconnect, which, by adopting a random graph topology, yields itself naturally to incremental expansion. Somewhat surprisingly, Jellyfish is more cost-efficient than a fat-tree: A Jellyfish interconnect built using the same equipment as a fat-tree, supports as many as 25% more servers at full capacity at the scale of a few thousand nodes, and this advantage improves with scale. Jellyfish also allows great flexibility in building networks with different degrees of oversubscription. However, Jellyfish's unstructured design brings new challenges in routing, physical layout, and wiring. We describe and evaluate approaches that resolve these challenges effectively, indicating that Jellyfish could be deployed in today's data centers.

==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We study the performance of \sys in different setups. With ns2, 
we study the performance of \sys in packet-level simulation~(\S\ref{sec:ev:pls}). 
Then we study the performance in flow-level simulation by modeling it 
as the multi-commodity max-flow problem~(\S\ref{sec:ev:fls}).

\vspace{-8pt}
\subsection{Packet Level Simulation}\label{sec:ev:pls}
\vspace{-8pt}


Apart from the previously discussed theoretical bounds on path lengths (Fig.~\ref{fig:pathlength}) and
bisection bandwidth (Fig.~\ref{fig:bisectionBound}), we present here preliminary 
results on the goodput of \sys in various configurations using discrete event simulation.

We use ns2 to simulate the goodput of \sys. 
The traffic matrix is a \emph{random permutation} of servers, such that each
server is sending traffic to just one other server and receiving traffic from
just one other server. 
We use fixed-sized packets in our workload.
Again, we evaluate \sys and fat-tree as the baseline for comparison.
We use ECMP to route via multiple shortest paths.

\begin{figure}[!t]
\centering
\subfigure[]{ \label{fig:ev:tcp}\includegraphics[width=2.9in]{figures/throughput}}
%\hspace{12pt}
\vspace{-8pt}
\subfigure[]{ \label{fig:ev:udp}\includegraphics[width=2.9in]{figures/throughputudp}}
%\subfigure[]{ \label{fig:plall}\includegraphics[width=2.2in]{figures/plall}}
\caption{\small \em Simluation results for \sys and fat-tree under random permutation traffic using (a) TCP and (b) UDP. 
We plot the goodput versus the number of servers supported while fixing the network cost for each curve.
}
%, and (c) the network diameter versus the number of servers.}
\label{fig:ev}
\vspace{-12pt}
\end{figure}

In Fig.~\ref{fig:ev:tcp}, we show the TCP goodput as the number of servers supported is increased.
We keep the network cost (total number of ports) constant for each curve we plot by changing the 
number of ports for servers/network. We observe that for any given cost, Jellyfish could provide considerably more design points, 
allowing potential expansion. As compared with fat-tree, Jellyfish could provide significantly higher TCP goodput or support 
a larger number of servers.

Fig.~\ref{fig:ev:udp} shows the goodput comparison under UDP. 
Without congestion control and packet reordering issues, fat-tree could achieve $\sim$$95\%$ of full bisection rate. 
However, \sys does not do as well as the fat-tree in this scenario. From simulation, 
we observed that some links have very low utilization. This reveals that ECMP might not be a good choice for \sys, especially 
in a smaller scale network. Therefore, we plan to modify ECMP to route through suboptimal paths.

\subsection{Flow Level Simulation}\label{sec:ev:fls}
TCP and routing inefficiencies do not allow for a raw comparison
of topology properties. Recent work has discussed overcoming
these problems through use of multipath TCP~\cite{mptcp} and
centralized routing controllers~\cite{microte}. Thus, to assess
the raw topology capabilities, we use a flow-level simulation
assuming optimal routing (based on solving the multi-commodity
flow problem using CPLEX). We compare the aggregate throughput
achieved by fat-tree topologies at various sizes and the best-known
degree-diameter graphs with \sys topologies built using the
exact same network equipment in each case. We use random server-level 
permutation traffic throughout.

%Ankit will do this
\subsubsection{Comparison with Best Known Degree-Diameter Graphs}

There is a fundamental trade-off between the degree and diameter of a 
graph of a fixed vertex-set (say of size $N$). At one extreme of this trade-off, is a clique --
maximum possible degree ($N - 1$), and minimum possible diameter ($1$).
At the other extreme is a disconnected graph with degree $0$ and diameter 
$\rightarrow \infty$. The problem of packing the maximum possible number
$N$ of nodes in a graph of fixed diameter and degree has 
received fair attention in graph theory. Even so, the optimal values
are only known for graphs of very small sizes (the largest degree-diameter
graph known to be optimal is of size $50$, with degree $7$ and diameter $2$).

The degree-diameter problem relates to our objective in that short average 
path lengths imply low resource usage and thus high network capacity.
Intuitively, the best known degree-diameter topologies should support a
large number of servers with high network bandwidth. We note that there
is a distinction between average path length (which relates more closely
to the network capacity) and the diameter. However, degree-diameter
graphs usually have small average path lengths too.

Thus, we use the best-known degree-diameter graphs as a benchmark for
comparison. Note that such graphs do not meet our incremental expansion
objectives. We merely use them to compare the raw topology capacity
(devoid of the burdens of routing and congestion control inefficiencies)
of \sys topologies.

The results of the comparison between \sys and degree-diameter graphs
are shown in Fig.~\ref{fig:ev:ddg}. In the worst of these
comparisons, \sys still achieves $\sim$$86\%$ of the degree-diameter
graph's aggregate throughput. In all other cases, \sys achieves over
$90\%$ of the degree-diameter graph's throughput. The number of
servers attached to the switches was decided such that full-bisection
bandwidth was not hit. (That would be unfair to the degree-diameter
graphs because they could still have additional capacity to support
some additional servers.)

Thus, not only is \sys incrementally expandable, it is close in 
network capacity to the best-known benchmarks.


\begin{figure}[!t]
\vspace{-12pt}
\centering
\includegraphics[width=3in]{figures/rndVsOpt}
\caption{\small \em Flow level simulation. \sys versus best-known degree-diameter graphs. 
x-axis label ($A$, $B$, $C$) represents the number of switches ($A$), the switch 
port-count ($B$), and the network degree ($C$). For y-axis, we normalized the throughput 
by the full bisection rate. Each bar compares the normalized throughput obtained by \sys
to that obtained by using the best-known degree-diameter graphs at that size using
the same network equipment and the same number of servers.
}
\label{fig:ev:ddg}
\end{figure}

%===================

\subsubsection{Comparison with Fat-tree}
In Fig.~\ref{fig:ev:fattree}, we show that starting at networks larger than $45$ switches, 
\sys can support a larger number of servers than an equal cost fat-tree at full line-rate. 
Using $180$ switches with $12$ ports each, the number of servers that \sys can support 
at the full line-rate is $\sim 26\%$ larger than that in a fat-tree built using the
same equipment. Also, this gap in the number of servers supported is steadily increasing
with the network size.

\begin{figure}[!t]
\vspace{-8pt}
\centering
\includegraphics[width=3in]{figures/mcf_fattree_comp}
\caption{\small \em Flow level simulation. \sys versus fat-trees: Given the same network equipments, we plot the number of servers can be supported in full sending rate under random permutation traffic.}
\label{fig:ev:fattree}
\vspace{-12pt}
\end{figure}


%===================

%Chi-Yao will do this.




==> incremental.tex <==
\section{Incremental Expansion}
\label{sec:increment}


Given an RRG($N$, $k$, $r$) topology, we would like to 
expand it to add more servers or/and increase the network
bisection bandwidth (if it's not full). In addition, we
\ankitb{MOVE TO INTRO AS A 'RESULT': would like to restrict rewiring as much as possible,
avoid replacing the network equipment in use, cause 
as little disruption to operations during the upgrade as possible,
and maintain the desirable properties: high bandwidth and
short paths at low cost.}

Say we restrict ourselves to the same $k$ and $r$, i.e. the
resulting topology RRG($N'>N$, $k$, $r$) uses the same 
port-count on its switches, with the same number of ports $r$
used for the network, and the rest used for servers. In other
words, we are adding identical racks complete with their servers 
and the ToR switch to the existing network. Then we can easily
expand from $N$ to $N'$ while preserving the bisection bandwidth
and the cost per server. To add one rack to the network, 
pick a random edge such that this ToR is not
already connected with either end-point, break this edge, 
and connect both end-points to the new ToR. This process 
can be repeated until no longer possible ($0$ or $1$ remaining 
network-ports on the new ToR). Repeat this procedure for as many 
new racks as desired. As noted in \S\ref{sec:topology},
the bisection bandwidth does not change between $N$ and $N'$.

Now say that we started out with a network with lower
capacity and want to increase the bisection
bandwidth of the network. The key here, is to use a similar
procedure as above, but without any servers being attached to the
new switches added (so we don't add racks, only the switches).
To maintain the $r$-regular property, we
can add $r$-port switches instead of $k$ and connect all
their ports to the network. (This network can no longer be
described as an RRG($N'$, $k$, $r$) because some switches
have no servers. It is still however, a $r$-regular
random graph at the switch layer.)

Further, given that $k$-port switches are already being
used in the network, we can continue to use the same switches
for expansion and connect all their $k$ ports to the network
using the same procedure as above. This is always strictly
better than our $r$-port switch based expansion. If
switches with even higher port-count are available, they can
be used similarly. Thus, \sys allows for heterogeneous expansion 
-- as new equipment with higher port-counts becomes available,
it can be readily used.

\ankitb{We note that our expansion procedures may not produce uniform-random 
RRGs. Verifying that the expanded topologies maintain the desirable
properties is the subject of future research.}


==> randomness.tex <==
\section{Moar Randomness!}
\label{sec:swdc}

In this section, we discuss related work that shares some parallels
with ours, while also being very different along several key design
ideas: Small-World Datacenters (SWDC)~\cite{swdc}\footnote{The record 
indicates that this work has been done in parallel to ours, as
evidenced by our HotCloud 2011 workshop paper.}. The SWDC design is
guided by the primary motivation of supporting key-value stores,
\ankitx{(how does this matter? Key-value stores have more locality?)}
and is based on using a regular lattice of servers, with a few random
links chosen in a small world manner (with probability of choosing
a neighbor decaying inversely in the dimension of the lattice with
the lattice-distance).

The SWDC proposal is not geared towards full-bisection bandwidth
topologies, as is clear from the server-centric design. With
a few ports per server, even the best-known degree-diameter
graphs will not provide full bisection bandwidth beyond a few
thousand servers.

Also, the use of a regular lattice underlying the topology creates
familiar problems with incremental expansion. For instance, using
a $2D$-Torus as the lattice implies that maintaining the network
structure when expanding an $n$ node network, requires addition of 
$2\sqrt n - 1$ new nodes. The higher-dimensional the lattice, the 
more complicated expansion becomes.

Such problems, of course, do not arise with a one-dimensional
lattice: the ring. But, they also do not arise with no lattice at
all. In addition, we show here that \sys topologies have higher 
network capacity under the random-permutation traffic model.
\ankitx{People might argue a little that this is not the `correct'
model to use.}

\ankitx{Add SWDC figure here on Sunday!}

Based on the trend shown in Fig.~\ref{fig:swdc}, we can safely
conclude that under this traffic model, that more (and uniform) 
randomness is better!


==> researchchall.tex <==
\section{Research Challenges}
\label{sec:challenges}
%\vspace{-7pt}

While random network topologies offer significant opportunities 
in flexibility, incremental expansion, and efficiency, they represent a dramatic departure from past 
data center network architectures, putting forth several challenges.

\paragraphb{Routing:} While structure has been the lead villain in our
story so far, it lends itself to simple and efficient routing
schemes. However, techniques such as spanning trees, which are 
used in switched networks, are not applicable to other 
recently proposed architectures either, because they do not 
exploit path diversity. Fat-tree-like 
topologies can benefit from Valiant Load Balancing over 
ECMP~\cite{vl2} but even there, prior work has shown a gap 
of $\sim$$20\%$ from the optimal throughput~\cite{microte}.
This has led recent work to propose a centralized controller to 
route \emph{elephant} flows, and a randomization-based strategy 
for the \emph{mice}~\cite{microte, devoflow}. This should work 
well for \sys too; a quantitative study remains the subject
of future work.

\paragraphb{Debugging:} Given the overwhelming size and complexity of
data center networks, even structured topologies do not offer `easy'
debugging. This has prompted a trend towards automated 
debugging applicable to general topologies~\cite{miswirings}, from which
\sys will also benefit.


